On the Impact of Sampling on Deep Sequential State Estimation

State inference and parameter learning in sequential models can be successfully performed with approximation techniques that maximize the evidence lower bound to the marginal log-likelihood of the data distribution. These methods may be referred to as Dynamical Variational Autoencoders, and our specific focus lies on the deep Kalman filter. It has been shown that the ELBO objective can oversimplify data representations, potentially compromising estimation quality. Tighter Monte Carlo objectives have been proposed in the literature to enhance generative modeling performance. For instance, the IWAE objective uses importance weights to reduce the variance of marginal log-likelihood estimates. In this paper, importance sampling is applied to the DKF framework for learning deep Markov models, resulting in the IW-DKF, which shows an improvement in terms of log-likelihood estimates and KL divergence between the variational distribution and the transition model. The framework using the sampled DKF update rule is also accommodated to address sequential state and parameter estimation when working with highly non-linear physics-based models. An experiment with the 3-space Lorenz attractor shows an enhanced generative modeling performance and also a decrease in RMSE when estimating the model parameters and latent states, indicating that tighter MCOs lead to improved state inference performance.

==> paper_sections/background.tex <==

% ----------------------------------------------------------------------
% -------------------- SUBSECTION
% ----------------------------------------------------------------------
\subsection{Dynamical Variational Autoencoders}
%
%
The joint distribution of the considered generative model can be factorized as $p_{\boldsymbol{\theta}}(\mathbf{x},\mathbf{z}) = p_{\boldsymbol{\theta}}(\mathbf{z})p_{\boldsymbol{\theta}}(\mathbf{x}|\mathbf{z})$. The so-called inference network $q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})$ is a parametric conditional distribution with parameters ${\boldsymbol{\phi}}$ that approximates the generally intractable posterior distribution $p_{\boldsymbol{\theta}}(\mathbf{z}|\mathbf{x})$. 
%
The ELBO is derived by applying Jensen's inequality to the marginal log-likelihood as
%
\begin{align}
\label{eq:elbo1d}
    \begin{split}
  &\log p_{\boldsymbol{\theta}}(\mathbf{x}) 
  %
  \geq 
  %
  \mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})}\left[\log\frac{p_{\boldsymbol{\theta}}(\mathbf{x},\mathbf{z})}{q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})}\right]  
  %
  = 
  %
\mathcal{L}^{\text{ELBO}}(\boldsymbol{\theta}, \boldsymbol{\phi};\mathbf{x}) \\& = 
%
\mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})}\left[\log p_{\boldsymbol{\theta}}(\mathbf{x}|\mathbf{z})\right] - \text{KL}(q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})||p_{\boldsymbol{\theta}}(\mathbf{z})).
\end{split}
\end{align}
%
The ELBO is maximized with respect to both $\phi$ and $\theta$ to learn both the generative model and the inference network. This mazimization can be peformed efficiently using gradient-based methods by using the reparameterization trick~\cite{kingma_auto-encoding_2022}.
%
This bound depends on the Kullback–Leibler (KL) divergence between the variational distribution and the distribution of the latent states.
%
%
%The ELBO is split into two terms, which is beneficial, as splitting the ELBO into two terms allows to analytically estimate the KL distance between the two distributions, meaning that only one of the terms has to be learned via stochastic gradient descent (SGD), lowering the variance of the gradient estimates of the bound.
%
% With the reparameterization trick proposed in~\cite{kingma_auto-encoding_2022}, the randomness in the states is propagated to an auxiliary variable such as $\boldsymbol{\epsilon} \sim \mathcal{N}\left(\mathbf{0},\ \mathbf{I}\right)$. %$\boldsymbol{\epsilon} \sim \mathcal{N}\left(\mathbf{0},\ \mathbf{I}\right)$. 
%
%This allows us to calculate the gradients of the ELBO w.r.t. both ${\boldsymbol{\theta}}$ and ${\boldsymbol{\phi}}$. 
%
% An unbiased estimator of the ELBO gradients w.r.t. both ${\boldsymbol{\theta}}$ and ${\boldsymbol{\phi}}$ can be obtained by generating $k$ samples of $\boldsymbol{\epsilon}$ and applying a deterministic mapping. %as $\mathbf{z} = g_{\boldsymbol{\phi}}\left(\boldsymbol{\epsilon},\,\mathbf{x}\right)$, where $z$ is a differentiable and invertible transformation of $\boldsymbol{\epsilon}$, given ${\boldsymbol{\phi}}$ and $\mathbf{x}$.
%
%
When considering the extension to the temporal setting which characterizes the DVAEs, the ELBO may be factorized as
\begin{align}
%\hspace*{-0.48cm}
\label{eq:elbo_dvae}
    \begin{split}
  &\mathcal{L}^{\text{DVAE}}({\boldsymbol{\theta}}, {\boldsymbol{\phi}}; \mathbf{x}) = 
  \sum^{T}_{t=1} \mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(z_{1:t}|\mathbf{x})}\left[\log p_{\boldsymbol{\theta}}\left(x_t|x_{1:t-1}, z_{1:t}\right)\right] 
  %
  \\ & \hspace*{-0.48cm} - \sum^{T}_{t=1} \mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(z_{1:t-1}|\mathbf{x})}\left[\text{KL}\left(q_{\boldsymbol{\phi}}(z_t|z_{1:t-1},\mathbf{x}\right)||p_{\boldsymbol{\theta}}(z_t|x_{1:t-1},z_{1:t-1}))\right].
\end{split}
\end{align}

%With DVAEs, the inference model and the generative 
In the particular case of the DKF, conditional independence of measurements and a first-order semi-Markov model (i.e., separately modeled time intervals) are assumed, which results in the following objective function
\begin{align}
%\hspace*{-0.6 cm}
\label{eq:elbo_dkf}
    \begin{split}
  &\mathcal{L}^{\text{DKF}}({\boldsymbol{\theta}}, {\boldsymbol{\phi}}; \mathbf{x}) = 
  \sum^{T}_{t=1} \mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(z_{t}|\mathbf{x})}\left[\log p_{\boldsymbol{\theta}}\left(x_t|z_t\right)\right]
  %
  \\ & - \text{KL}(q_{\boldsymbol{\phi}}(z_1|\mathbf{x})||p_0(z_1))
  %
  \\ & - \sum^{T}_{t=2} \mathop{\mathbb{E}}_{q_{\boldsymbol{\phi}}(z_{t-1}|\mathbf{x})}\left[\text{KL}\left(q_{\boldsymbol{\phi}}(z_t|z_{t-1},\mathbf{x}\right)||p_0(z_t|z_{t-1}))\right].
\end{split}
\end{align}



%
Let us consider the dataset $\mathcal{D} = \{\mathbf{x}^{(i)}\}^{N}_{i=1}$ with $N$ i.i.d. datapoints corresponding to samples of the continuous variable $\mathbf{x}$.
%
The expectation in~\eqref{eq:elbo_dkf} can be approximated using Monte Carlo integration, leading to the DKF approximated objective for the lower bound on the marginal likelihood of datapoint $\mathbf{x}^{(i)}$ as
%
\begin{align}
%\hspace*{-0.6 cm}
\label{eq:mc_approx_dkf}
    \begin{split}
  &\tilde{\mathcal{L}}^{\text{DKF}}_K({\boldsymbol{\theta}}, {\boldsymbol{\phi}}; \mathbf{x}^{(i)}) = 
  %
  \frac1{K}\sum_{k=1}^{K}\sum^{T}_{t=1} \log p_{\boldsymbol{\theta}}(x_t^{(i)}|z_t^{(k)} )
  %
  \\ & 
  - \text{KL}(q_{\boldsymbol{\phi}}(z_1|\mathbf{x})||p_0(z_1))
  %
  \\ & 
  - \frac1{K}\sum_{k=1}^{K}\sum^{T}_{t=2}\text{KL}(q_{\boldsymbol{\phi}}(z_t|z_{t-1}^{(k)},\mathbf{x}^{(i)})||p_0(z_t|z_{t-1}^{(k)})),
\end{split}
\end{align}
%
%where \cred{ $z_t^{(k)} = g_{\boldsymbol{\phi}}(\epsilon_t^{(k)}, z_{t-1},\mathbf{x}^{(i)})$.} 
%
\cred{[RB: is $\beta$ annealing fact.? I'd remove it from here and mention just in the experimental setting, in text. I'd also use capital K for the number of MC samples (or maybe L, there are two MC samplings that take place, one w.r.t. x here, and one later, w.r.t. the importance samples), to keep consistent with N and T (capital italics = constants)] [HC: Done]}
where $k$ is the Monte Carlo sample index. This expression can be simplified by introducing the unnormalized logarithmic weights as $w^{(i,k)} = w(\mathbf{x}^{(i)},\mathbf{z}^{(k)},{\boldsymbol{\theta}}) = p_{\boldsymbol{\theta}}(\mathbf{x}^{(i)},\mathbf{z}^{(k)})/q_{\boldsymbol{\phi}}(\mathbf{z}^{(k)}|\mathbf{x}^{(i)})$. The unbiased estimator of the DKF objective function can then be calculated as
%
%After using the reparameterization trick and by drawing $k$ samples of the auxiliary variable $\boldsymbol{\epsilon} \sim \mathcal{N}\left(\mathbf{0},\ \mathbf{I}\right)$ (please refer to~\cite{kingma_auto-encoding_2022, burda_importance_2016} for the notation), the expectation of the objective gradients can be computed with Monte Carlo as
%
\begin{equation}
\label{eq:monte_carlo_vae}
    \nabla_{\boldsymbol{\theta}}\tilde{\mathcal{L}}_K^{\text{DKF}}({\boldsymbol{\theta}}, {\boldsymbol{\phi}}; \mathbf{x}^{(i)}) =  \frac{1}{K}\sum_{k=1}^{K}\nabla_{\boldsymbol{\theta}} \log w_{\text{DKF}}^{(i,k)},
\end{equation}
%
where $w_{\text{DKF}}$ includes the objective function factorization as given by the DKF.
%
%
%
%
This expression would also apply to the general DVAE case if the unnormalized importance weights $w_{\text{DVAE}}$ were calculated considering the factorization in \eqref{eq:elbo_dvae}.
%
%By estimating ${\boldsymbol{\theta}}$ (i.e., the generative model parameters), we gain knowledge on the transition and emission models, which allow to build the states from the latent space and also the observations. The importance weighting approach can be applied regardless of the assumed distribution. However, assuming that the latent states are normally distributed is to some extent necessary because the reparameterization trick that appears in VAEs only works for certain distributions, holding for the exponential family but breaking for discrete distributions. This would be a limitation to take into account when using a VAE architecture in structured inference networks which require the use of different distributions. However, as the aim of this paper is to assess whether importance sampling can help with dynamical models and our benchmark is the algorithm provided in~\cite{krishnan_structured_2016}, we consider it necessary to follow their same assumptions.


% ----------------------------------------------------------------------
% -------------------- SUBSECTION
% ----------------------------------------------------------------------
% \subsection{Expectation Maximization and VAEs}


% ----------------------------------------------------------------------
% -------------------- SUBSECTION
% ----------------------------------------------------------------------
\subsection{Importance Weighted Autoencoders}
%
Monte Carlo Objectives (MCOs) generalize the ELBO to objectives defined by taking the log of a positive, unbiased estimator of the marginal log-likelihood as
%
%$\log p_{\boldsymbol{\theta}}(\mathbf{x})$, being this estimator denoted as $\hat{p}_N(\mathbf{x})$. The MCO over the joint density $p_{\boldsymbol{\theta}}(\mathbf{x}, \mathbf{z})\in\mathcal{P}$ is defined as
%
\begin{equation}
    \mathcal{L}(\mathbf{x}) = \mathbb{E}[\log\hat{p}_N(\mathbf{x})].
\end{equation}
%
%In~\cite{maddison_filtering_2017}, they show how the tightness of an MCO is closely related to the variance of the estimator defining it. There are multiple works proposing tighter bounds than the ELBO, such as the importance weighted autoencoder (IWAE) and particle-based MCOs such as the so-called filtering variational objectives (FIVOs)~\cite{maddison_filtering_2017}. 
%
As emphasized in Section~\ref{sec:intro}, the tightness of an MCO is related to the variance of $\hat{p}_N(\mathbf{x})$~\cite{maddison_filtering_2017} and consequently there are multiple works proposing alternative objective functions that are tighter than the ELBO. 
%
We focus on the IWAE bound, which is derived from the $K$-sample importance weighting estimate of the marginal log-likelihood as
%
%The IWAE bound takes the estimator of the marginal log-likelihood without extension to the temporal setting to be $N$ averaged i.i.d. importance weights of the marginal log-likelihood.
%
%
%This objective is introduced as
%
\begin{equation}
\label{eq:iwae_bound}
    \mathcal{L}_K^{\text{IWAE}}(\boldsymbol{\theta}, \boldsymbol{\phi}; \mathbf{x}) = \mathbb{E}_{\mathbf{z}_1,\,\hdots,\,\mathbf{z}_K\sim\,q_{\boldsymbol{\phi}}(\mathbf{z}|\mathbf{x})}\left[\log\frac{1}{K}\sum_{k=1}^{K}w_{\text{VAE}}^{(k)}\right],
\end{equation}
%
where $\mathbf{z}_1,\,\hdots,\,\mathbf{z}_K$ are sampled independently from the recognition model and $w_{\text{VAE}}$ considers the non-dynamical structure from a regular VAE. 
%
%
%
%The normalized importance weights are denoted as $\tilde{w_i}=w_i/\sum_{i=1}^k w_i$ and show in the following derivations.
%
It has been shown that this bound is tighter for an increasing number of importance weighting samples~\cite[Appendix A]{burda_importance_2016}, which can be deduced from the properties of Monte Carlo integration. This enables the learning of richer data representations with more latent dimensions, which translates into significantly higher log-likelihoods on density estimation benchmarks. 
%

%The VAE objective heavily penalizes the samples from the approximate posterior that fail to explain the observations, thus placing a strong constraint on the model. On the other hand, with the IWAE~\cite{burda_importance_2016}, the trained generative network has a posterior distribution that does not fit the VAE assumptions, thus providing additional flexibility. 
%

\cred{[RB: maybe we discussed this in a meeting, I can't remember, but it could be better to move the following subsection already to section 3, so you explain the MCOs, IWs, etc. directly on the dynamical model case, this would also highlight more the contribution of the paper. You could also remove some redundancy this way, because all the eqs. that are for the (IW)VAE in the next subsection will already be directly to the DKF, so 11 may not be needed, as you can go directly to 12 ] [HC: Discuss in meeting]}

==> paper_sections/experimental_setup.tex <==
\subsection{Learning DMMs with Polyphonic Music Data}
%
The DKF framework proposed in~\cite{krishnan_structured_2016} serves as our benchmark, and we adapt its objective function to align with the method in Section~\ref{sec:iw-dkf}. For this experiment, most settings are consistent with the ones in~\cite[Polyphonic Music Experiment]{krishnan_structured_2016}. The inference network $q_{\phi}(z_t|z_{t-1}, \mathbf{x})$ is fixed and includes an RNN and a combiner function. We learn a DMM on a polyphonic music dataset, where an instance in the sequence $x_t \in \mathbb{R}^{88}$ comprises an 88-dimensional binary vector corresponding to the notes of a piano. The KL divergence is annealed in the objective function from 0 to 1 over 5000 parameter updates. Results are reported based on early stopping using the validation set. For the testing set, an importance sampling-based estimate of the NLL is provided following~\eqref{eq:ll_estimate} considering the samples in $\mathcal{D}_{\text{test}} \subseteq \mathcal{D}$. The latent states in this dataset $z_t \in \mathbb{R}^{100}$ do not have a physical meaning and consequently it is not possible to evaluate state estimation performance for this experiment. Acknowledging this limitation, in the next experiment the framework is accommodated to address sequential state and parameter estimation when working with highly non-linear physics-based models.

\begin{comment}
\subsection{Linear Gaussian Model}
%
Regarding parameter estimation, if the model is Gaussian linear, we can compute the parameter posterior in c-f. And then, as direct evaluation of the posterior is feasible, we can get the parameter estimate with ML/MAP, or MCMC methods. We compare the following methods:
%
\begin{itemize}
    \item IWAE (maybe we try for different values of $k$)
    \item Kalman Filter
    \item Kalman Smoother
    \item Expectation Maximization (Sarkka chapter 12)
\end{itemize}
\end{comment}



\subsection{State Estimation with a Physics-based Model}
%
\cred{[HC: Tales you can cite your paper with Ahmet somewhere: ~\cite{2022_fusion_lorenz}]}.
For this experiment, we consider the 3-space Lorenz attractor~\cite{Lorenz1963DeterministicNF} as an example of a non-linear chaotic system. In this case, the parametric form of the mean and covariance of the transition and emission models are known, and this allows us to analyze the IW-DKF performance in terms of state estimation. This model consists of three ordinary differential equations and can be discretized as
\begin{align}
\begin{split}
&z_t = z_{t-1} + T_s f(z_{t-1}) + q_t \\
%
&x_t = z_t + r_t
\end{split}
\end{align}
%
where $z_t \in \mathbb{R}^3$ and $x_t \in \mathbb{R}^3$ are the latent state and observation at time instant $t$ and $\boldsymbol{\theta} = \{\sigma,\, \rho,\, \beta\}$ are the generative model parameters. The vector valued function $f(\cdot) = [f_1(\cdot), f_2(\cdot), f_3(\cdot)]^\top$ represents the dynamical model as
%
\begin{align}
\begin{split}
    f_1({z}_{t}) & = \sigma (z_{t,2} - z_{t,1})
    \numberthis \label{eq:lorenz_z1} \\
    f_2({z}_{t}) & =  z_{t,1} (\rho - z_{t,3}) 
    \numberthis \label{eq:lorenz_z2} \\
    f_3({z}_{t}) & = z_{t,1} z_{t,2} -  \beta z_{t,3}
    \numberthis \label{eq:lorenz_z3}.
\end{split}
\end{align}
%
%
In the experiments, the state and measurement noise was set to $r_t,\, q_t \sim \mathcal{N}(\mathbf{0}, 0.1\,\mathbf{I})$
%
The initial state was set to $\mathbf{z}_0 = (1, 1, 1)^\top$, and the generative model parameters as $\sigma=28$, $\rho=10$, and $\beta=8/3$, and $T_s = 0.1$s. 
%



==> paper_sections/method_deprecated.tex <==
If we compare equations~\eqref{eq:monte_carlo_vae} and~\eqref{eq:monte_carlo_iwae}, we can see that the difference between them relies on the normalized weights coefficient $\tilde{w_i}$. This suggests that applying IS to VAEs can be done in a straightforward manner, just by adding this normalized constant in the objective. However, the challenge can appear when using sequential methods, as the model is extended to the temporal setting and thus Markovian and conditional independence assumptions need to be applied to efficiently perform inference.
%
%In Section~\ref{subsec:method_comparison}, we compare the structured inference and deep kalman filter methods, which are extended to the temporal setting, to IWAEs, which allows us to accurately describe how we merge the two approached in Section~\ref{subsec:proposed_method}.
%
%
%\begin{figure}[h]
 %   \centering
 %       \caption{Comparison method between (a) the methods in~\cite{krishnan_structured_2016} and~\cite{krishnan_deep_2015}, on structured inference of the posterior of complex sequential models - which make use of VAEs, and (b) the IWAE framework~\cite{burda_importance_2016}.}
  %  \label{results:sanity_check}
    % \includegraphics[width=0.8 \textwidth]{Figures/Results/November_classification_results/classification_oroville_dam_1_epsilon_0.05_norm_constant_0.3_selected_dates.pdf}
   % \includegraphics[width=9cm]{figures/characteristics_table.png}
   % \label{fig:comparative}
%\end{figure}
%
%
%\subsection{DKF vs. IWAEs}
%\label{subsec:method_comparison}
%In this subsection, we highlight the differences between (a) the methods in~\cite{krishnan_structured_2016} and~\cite{krishnan_deep_2015}, on structured inference of the posterior of complex sequential models - which make use of VAEs, and (b) the IWAE framework~\cite{burda_importance_2016}. These differences are clearly stated in Figure~\ref{fig:comparative}.
%
\\

%
%Although this subsection aims to highlight the differences between the methods, we start with the similarities between (a) and (b). Both methods use unbiased estimates of the MCO gradients (not specifically the ELBO objective). This is well explained in~\cite{maddison_filtering_2017}. Furthermore, both approaches use the same architecture (a generative network, with the generative model parameters $\theta$ and a recognition network or variational distribution, with the variational parameters $\phi$). Also, in (a) and (b) they consider the same modeling assumptions: the recognition model must be inside the Gaussian family for the VAE or IWAE, which allows to properly represent the states given that they are assumed to be Gaussian as well.
%
\\

%
%Regarding the differences between (a) and (b), in the case of (a), 
On the one hand, the VAE update from the DKF computes the gradients w.r.t. $\theta$ and $\phi$, leading to lower variance gradient estimates. This is possible only thanks to the reparameterization trick, which can only be applied when the underlying model is differentiable. These gradients are also referred to as the reparameterization gradients. On the other hand, the IWAE update is closer to a REINFORCE-like update rule~\cite[Section 2.9.1]{kingma_introduction_2019}, which only computes the gradients w.r.t. $\theta$. In this case, the objective function cannot be separated into two terms, i.e., the KL divergence and the underlying log-likelihood model, which leads to higher variance gradient estimates. This happens when the model is not differentiable. However, we still need to work with an evaluable model in order to compute the score gradients.
%
The reason why score gradients have a higher variance is that the stochastic gradient descent update is performed for the whole objective, unlike with the reparameterization gradients, where the KL is computed analytically and the only term being optimized via updates is the log-likelihood of the underlying model. High variance estimates are not of our interest because they make algorithm convergence difficult. When that happens, there are several techniques that can be used to overcome the issue, such as lowering the step size, or learning rate, which makes convergence very slow, or the use of variance reduction methods such as control variates~\cite{ranganath_black_2013}.
%
%


The posterior distribution in the DKF is factorized by considering the first-order Markov and the conditional independence assumptions~\cite[Section 4.1]{särkkä_2013}.
%
Considering this, the importance weights may be factorized as
%
\begin{align}
    \begin{split}
    &\sum_i w_i = \sum_i \frac{p(\vec{\mathbf{x}}|\vec{\mathbf{z}_i})p(\vec{\mathbf{z}_i})}{q(\vec{\mathbf{z}_i}|\vec{\mathbf{x}})} \\&= \sum_i\frac{p(z_{i,1})p(x_1|h_{i,1})\Pi^T_{t=2}p(x_t|z_{i,t})p(z_{i,t}|z_{i,t-1})}{ q(z_{i,1}|x_{1:T})\Pi^T_{t=2}q(z_{i,t}|h_{i,t-1}, x_{t:T})}.
\end{split}
\end{align}
%
%    &\sum_i w_i = \sum_i \frac{p(\vec{\mathbf{x}}|\vec{\mathbf{z}_i})p(\vec{\mathbf{z}_i})}{q(\vec{\mathbf{z}_i}|\vec{\mathbf{x}})} \\&= \sum_i \frac{p(z_{i,1})\Pi_{t=1}^Tp(x_t|z_{i,t})p(z_{i,t}|z_{i,t-1})}{q(\vec{\mathbf{z}_i}|\vec{\mathbf{x}}) = q(z_{i,1}|x_{1:T})\Pi^T_{t=2}q(z_{i,t}|h_{i,t-1}, x_{t:T})},
%
%while the factorization of the posterior can be expressed as
%
%\begin{equation}
 %   q(\vec{\mathbf{z}_i}|\vec{\mathbf{x}}) = q(z_{i,1}|x_{1:T})\Pi^T_{t=2}q(z_{i,t}|h_{i,t-1}, x_{t:T}),
%end{equation}
%
%which leads to the final expression of the importance weights summation 
%
%\begin{equation}
 %    \sum_i w_i = \sum_i\frac{p(z_{i,1})p(x_1|h_{i,1})\Pi^T_{t=2}p(x_t|z_{i,t})p(z_{i,t}|z_{i,t-1})}{ q(z_{i,1}|x_{1:T})\Pi^T_{t=2}q(z_{i,t}|h_{i,t-1}, x_{t:T})}.
%\end{equation}
%
%
%
In this project we do not leverage the temporal dimension of the data and states, but directly apply importance weighting to the MCO. Consequently, the objective function is the same as the one of the IWAEs, but with an addition that consists in applying the Markovian and conditional indepence assumptions to the posterior. This is challenging given the summation in the importance weighting sample average from the IWAE objective. 
%
\subsection{Approach used to introduce the weights}
The question assessed in this subsection relies on finding the best way to introduce the importance weights in the DKF update function. We pose both strategies and explain why the second one is the one we selected.
%
%
%

\textbf{Approach 1.} The first approach consists in applying the importance weights at the bound level. This would correspond to adding $w_i$ and $\tilde{w_i}$ in the structured inference and deep Kalman filter models in their step equivalent to Equation~\eqref{eq:iwae_bound}. 
%
%

\textbf{Approach 2.} The second approach consists in applying the importance weights directly when reaching the equivalent training stage, meaning Equation~\eqref{eq:monte_carlo_iwae}. This approach can be followed in two ways, the first one (2.a) being applying the extension to temporal setting, Markovity and conditional independence both to $w_i$ and $\tilde{w_i}$ and the second one (2.b) being more straightforward and only related to the normalized importance weights.
%

%
We believe that approach 1 can actually not be performed given the summation in the average $\hat{p}_N(x)$, so this approach is discarded. We believe however that approach 2 is feasible, being 2.b) more straightforward than 2.a), as 2.b) can be performed by only computing the normalized weight and multiplying them by the VAE update in Equation~\eqref{eq:monte_carlo_vae}. Consequently, we decide to follow approach 2.b), where we compute the normalized weights for each drawn sample $k$ and multiply by the loss term corresponding to that sample. The gradients are commputed and cumulated for each of the drawn samples as well. Equations (10)-(12) are used to implement this approach.
\label{subsec:proposed_method}
%

==> paper_sections/results.tex <==
\subsection{Experiment 1: DMMs}
The training and test log-likelihood for the DKF and the IW-DKF for $k = 1,\, 5,\, 15$ when tested on the polyphonic music dataset are shown in Figure~\ref{fig:results_poly}. Table~\ref{table:results_poly} shows the mean and standard deviation (in parentheses) of the log-likelihood (training, validation and test) and KL divergence (training and validation) for the IW-DKF for $k = 1,\, 5,\, 15$ also when training on a DMM with the polyphonic music dataset.

\begin{figure}[]
\includegraphics[width=0.95\linewidth]{figures/results/polyphonic/poly_train_test_bound.pdf}
\vspace{-4ex}
\caption{Training (upper plot) and test (lower plot) log-likelihood for the DKF~\cite{krishnan_deep_2015,krishnan_structured_2016} and the IW-DKF for $k = 1,\, 5,\, 15$ when tested on the polyphonic music dataset.}
\label{fig:results_poly}
\end{figure}



For a given probability measure $\mu$ on $\mathbb{R}^d$, we denote $\mu \in \mathcal{P}_2(\mathbb{R}^d)$ if its second moment is finite.


\begin{comment}
\begin{table}[]
\begin{tabular}{cllllllll}
\hline
\multicolumn{1}{l}{} & \multicolumn{3}{c}{LL}                                                                & \multicolumn{2}{c}{KL}                                     & \multicolumn{3}{c}{NLL}                                                               \\ \hline\hline
k                    & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} \\ \hline
1                    & -0.865 (0.029)            & -0.888 (0.041)                 & -7.795 (0.339)           & 0.045 (0.006)             & 0.047 (0.012)                  & 1.495 (0.023)             & 1.451 (0.025)                  & 7.791 (0.349)            \\ \hline
5                    & -0.853 (0.008)            & -0.876 (0.007)                 & -7.513 (0.183)           & 0.044 (0.002)             & 0.045 (0.002)                  & 1.503 (0.013)             & 1.463 (0.013)                  & 7.506 (0.2)              \\ \hline
15                   & -0.848 (0.008)            & -0.875 (0.007)                 & -7.485 (0.159)           & 0.043 (0.002)             & 0.044 (0.002)                  & 1.509 (0.013)             & 1.459 (0.014)                  & 7.489 (0.169) \\ \hline
\end{tabular}
\end{table}
\end{comment}


\addtolength{\tabcolsep}{-3pt}
\centering
\begin{table}[]
\fontsize{7.5}{8}\selectfont
\begin{tabular}{clllll}
\\ \hline
\multicolumn{1}{l}{} & \multicolumn{3}{c}{{\ul LL}}                                                          & \multicolumn{2}{c}{{\ul KL}}                               \\ \hline\hline
k                    & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} & \multicolumn{1}{c}{Test} & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} \\ \hline
1                    & -0.865 (0.029)            & -0.888 (0.041)                 & -7.795 (0.339)           & 0.045 (0.006)             & 0.047 (0.012)                  \\ \hline
5                    & -0.853 (0.008)            & -0.876 (0.007)                 & -7.513 (0.183)           & 0.044 (0.002)             & 0.045 (0.002)                  \\ \hline
15                   & -0.848 (0.008)            & -0.875 (0.007)                 & -7.485 (0.159)           & 0.043 (0.002)             & 0.044 (0.002)                 \\ \hline
\end{tabular}
\caption{Mean and standard deviation (in parentheses) of the log-likelihood (training, validation and test) and KL divergence (training and validation) for the IW-DKF for $k = 1,\, 5,\, 15$ when training on a DMM with the polyphonic music dataset. Values have been calculated considering results in Figure~\ref{fig:results_poly} after convergence, i.e., epoch 350 approximately.}
\label{table:results_poly}
\end{table}


\cred{[for the tables, I would remove the horizontal lines between the different k to clean them up a bit]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Linear Gaussian Model}
The expectation maximization (EM) algorithm alternatively optimizes the ELBO w.r.t $\phi$ and $\theta$ in the expectation and maximization steps, respectively. It has been shown that the encoder-decoder architecture of the VAE can be suboptimal~\cite{he2019lagging}.
\end{comment}

\subsection{Chaotic System}
In Figure~\ref{fig:results_chaotic_oneMCrealization}, results for one Monte Carlo realization are shown.
%
\begin{figure}[]
\centering
\includegraphics[width=0.75\linewidth]{figures/results/chaotic/chaotic_trajectory_700.pdf}
\caption{(Upper plot) 3D Lorenz attractor trajectory for one datapoint with $T = 100$ from the validation set. True and estimated states with the IW-DKF for $k = 1,\, 5$ are shown for this specific trajectory. (Lower plot) RMSE in the states with the IW-DKF for $k = 1,\, 5$ for the whole validation set in one scenario.}
\label{fig:results_chaotic_oneMCrealization}
\end{figure}


% \addtolength{\tabcolsep}{-3pt}
\centering
\begin{table}[]
\fontsize{8.3}{9.5}\selectfont
\begin{tabular}{clllll}
\\ \hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{{\ul LL}}                                                          & \multicolumn{2}{c}{{\ul KL}}                               \\ \hline\hline
k                    & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation}  & \multicolumn{1}{c}{Train} & \multicolumn{1}{c}{Validation} \\ \hline
1  & -2.61 (0.13)     & -2.63 (0.13)          & 5.1 (1.05)      & 5.2 (0.96)                  \\ \hline
5    & -1.94 (0.02)   & -1.92(0.026)    & 4.64 (0.39)   & 4.34 (0.35)                  \\ \hline
\end{tabular}
\caption{Mean and standard deviation (in parentheses) of the log-likelihood (training, validation and test) and KL divergence (training and validation) for the IW-DKF for $k = 1,\, 5$ when training on a DMM with the polyphonic music dataset. Values have been calculated considering the scenario in Figure~\ref{fig:results_chaotic_oneMCrealization} after convergence, i.e., epoch 600 approximately.}
\label{table:results_chaotic_oneMCrealization}
\end{table}



